On the Complexity of Secluded Path Problems

This paper investigates the complexity of finding secluded paths in graphs. We focus on the \textsc{Short Secluded Path} problem and a natural new variant we introduce, \textsc{Shortest Secluded Path}. Formally, given an undirected graph $G=(V, E)$, two vertices $s,t\in V$, and two integers $k,l$, the \textsc{Short Secluded Path} problem asks whether there exists an $s$-$t$ path of length at most $k$ with at most $l$ neighbors. This problem is known to be computationally hard: it is W[1]-hard when parameterized by the path length $k$ or by cliquewidth, and para-NP-complete when parameterized by the number $l$ of neighbors. The fixed-parameter tractability is known for $k+l$ or treewidth. In this paper, we expand the parameterized complexity landscape by designing (1) an XP algorithm parameterized by cliquewidth and (2) fixed-parameter algorithms parameterized by neighborhood diversity and twin cover number, respectively. As a byproduct, our results also yield parameterized algorithms for the classic \textsc{$s$-$t$ $k$-Path} problem under the considered parameters. Furthermore, we introduce the \textsc{Shortest Secluded Path} problem, which seeks a shortest $s$-$t$ path with the minimum number of neighbors. In contrast to the hardness of the original problem, we reveal that this variant is solvable in polynomial time on unweighted graphs. We complete this by showing that for edge-weighted graphs, the problem becomes W[1]-hard yet remains in XP when parameterized by the shortest path distance between $s$ and $t$.

==> preamble.tex <==
\ProvidesPackage{preamble}

\crefname{claim}{Claim}{Claims}

\usepackage[dvipsnames]{xcolor}
\usepackage{tcolorbox}

\usepackage{algorithm}
\usepackage{algpseudocode}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% -------------- todonotes ---------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% https://ctan.org/pkg/todonotes

\usepackage{todonotes}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% --------------- multicol ---------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%% https://www.ctan.org/pkg/multicol
%%%%%%%%%%%%%%%%%% https://stackoverflow.com/questions/1398127/breaking-a-list-into-multiple-columns-in-latex
\usepackage{multicol}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% -------------- standalone --------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage[mode=buildnew]{standalone}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% -------------- mathtools ---------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%% package
\usepackage{mathtools}
\usepackage{cite}

%%%%%%%%%%%%%%%%%% Paired Deliminets
\DeclarePairedDelimiter{\braces}{\{}{\}}            % for braces
\DeclarePairedDelimiter{\bracks}{[}{]}              % for brackets
\DeclarePairedDelimiter{\parens}{(}{)}              % for parentheses
%
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}       % for absolute value
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}      % for ceiling
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}   % for floor
\DeclarePairedDelimiter{\clip}{[}{]}                % for clipping
\DeclarePairedDelimiter{\negpart}{[}{]_{-}}         % for negative part
\DeclarePairedDelimiter{\pospart}{[}{]_{+}}         % for positive part
%
\DeclarePairedDelimiterX{\setdef}[2]{\{}{\}}{#1 : #2}        % for set builder notation
\DeclarePairedDelimiterXPP{\exclude}[1]{\mathopen{}\setminus}{\{}{\}}{}{#1}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% ----------------- tikz -----------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%% package
\usepackage{tikz}
\usetikzlibrary{shapes.geometric, positioning}
%%%%%%%%%%%%%%%%%% arrows and other
\usetikzlibrary{decorations,decorations.pathmorphing,decorations.pathreplacing,fit,positioning,arrows,calc,backgrounds,topaths}


%%%%%%%%%%%%%%%%%% white vertices 
\tikzstyle{vertex}=[circle, draw, inner sep=2pt,  minimum width=1 pt, minimum size=0.1cm]
%%%%%%%%%%%%%%%%%% black vertices 
\tikzstyle{black_vertex}=[circle, draw, inner sep=2pt, fill=black!100, minimum width=1pt, minimum size=0.1cm]
%%%%%%%%%%%%%%%%%%% gray vertices 
\tikzstyle{gray_vertex}=[circle, draw, inner sep=2pt, fill=lightgray, minimum width=1pt, minimum size=0.1cm]

\tikzset{
    fpt/.style={
        shape=rectangle,
        fill=green!40!white,
        draw,
        line width= .2,
        rounded corners = 3pt,
        inner sep = 2,
        outer sep = 2,
        minimum height = 12,
    },
    w1/.style={
        shape=rectangle,
        fill=orange!40!white,
        rounded corners = 3pt,
        inner sep = 2,
        outer sep = 2,
        minimum height = 12,
    },
    nph/.style={
        shape=rectangle,
        fill=red!40!white,
        rounded corners = 1pt,
        inner sep = 3,
        outer sep = 3,
        draw,
        double,
        double distance=1,
        minimum height = 12,
    }
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% --------------- apxproof ---------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%% https://github.com/PierreSenellart/apxproof
%%%%%%%%%%%%%%%%%% package
 \usepackage[bibliography=common]{apxproof} %(conf submission)
% % \usepackage[appendix=strip]{apxproof}  %remove the appendix (camera ready)
% % \usepackage[appendix=inline]{apxproof} %content in the main text (arxiv)


% % --- apxproof の設定 ---
% % 本文中で定理が再掲されることを示すマーク (★)
% \renewcommand{\mainbodyrepeatedtheorem}{\textup{($\star$)}}


% % --- apxproof を使った定理環境の定義 ---
% % カウンターの指定を正しく行う
% \newtheoremrep{theorem}[section]{Theorem}
% \newtheoremrep{lemma}[theorem]{Lemma}
% \newtheoremrep{claim}[theorem]{Claim}
% \newtheoremrep{corollary}[theorem]{Corollary}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -------------- problemdef --------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{boxedminipage}
\usepackage[normalem]{ulem}
% \usepackage[export]{adjustbox}
\usepackage{framed}
\usepackage{xspace}
\usepackage{xifthen}
\usepackage{tabularx}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ------------------------------------ COMMANDS ------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%% Some standard commands
\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}
\newcommand{\bO}{{\cal O}}
\newcommand{\tO}{\tilde{\bO}}
\newcommand{\sO}{\bO^{\star}}
\newcommand{\poly}{{\rm poly}}


\newcommand{\paramstyle}[1]{\text{\rm #1}}
\newcommand{\tw}{\paramstyle{tw}}
\newcommand{\nd}{\paramstyle{nd}}
\newcommand{\pw}{\paramstyle{pw}}
\newcommand{\td}{\paramstyle{td}}
\newcommand{\vc}{\paramstyle{vc}}
\newcommand{\mw}{\paramstyle{mw}}
\newcommand{\ml}{\paramstyle{ml}}
\newcommand{\fvs}{\paramstyle{fvs}}
\newcommand{\vi}{\paramstyle{vi}}
\newcommand{\cvd}{\paramstyle{cvd}}
\newcommand{\fes}{\paramstyle{fes}}
\newcommand{\cw}{\paramstyle{cw}}
\newcommand{\bw}{\paramstyle{bw}}
\newcommand{\ms}{\paramstyle{ms}}
\newcommand{\tc}{\paramstyle{tc}}
\newcommand{\mcc}{\paramstyle{mcc}}

\newcommand{\cc}{\text{\tt cc}}

\newcommand{\M}{\mathcal{M}}
\newcommand{\OPT}{\operatorname{OPT}}
\newcommand{\ALG}{\operatorname{ALG}}

\newcommand{\diam}{\operatorname{diam}}
\newcommand{\dist}{\operatorname{dist}}

\newcommand{\lab}{{\mathtt{lab}}}

%%%%%%%%%%%%%%%%%% Problem Definitions
\newcommand{\problemstyle}[1]{{\sc #1}}
\newcommand{\TB}{\problemstyle{Telephone Broadcast}}
\newcommand{\TBMS}{\problemstyle{Telephone Broadcast with Multiple Sources}}
\newcommand{\NMTS}{\problemstyle{Numerical Matching with Target Sums}}
\newcommand{\RNMTS}{\problemstyle{Restricted Numerical Matching with Target Sums}}



%%%%%%%%%%%%%%%%%% Spaces
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Nplus}{\N^+}
\newcommand{\Nzero}{\N_0}



%%%%%%%%%%%%%%%%%% Problem Definition Environment
\newlength{\RoundedBoxWidth}
\newsavebox{\GrayRoundedBox}
\newenvironment{GrayBox}[1]{
        \setlength{\RoundedBoxWidth}{.93\textwidth}
        \def\boxheading{#1}
        \begin{lrbox}{\GrayRoundedBox}
        \begin{minipage}{\RoundedBoxWidth}
    }{
        \end{minipage}
        \end{lrbox}
        \begin{center}
            \begin{tikzpicture}%
               \node(Text)[draw=black!20,fill=white,rounded corners,%
                     inner sep=2ex,text width=\RoundedBoxWidth]%
                     {\usebox{\GrayRoundedBox}};
                \coordinate(x) at (current bounding box.north west);
                \node [draw=white,rectangle,inner sep=3pt,anchor=north west,fill=white]
                at ($(x)+(6pt,.75em)$) {\boxheading};
            \end{tikzpicture}
        \end{center}
    }

\newenvironment{defproblemx}[2][]
    {
        \noindent\ignorespaces%
        \FrameSep=6pt%
        \parindent=0pt%
        \vspace*{-1.5em}
        \ifthenelse{\isempty{#1}}{%
            \begin{GrayBox}{\textsc{#2}}%
            }{%
              \begin{GrayBox}{\textsc{#2} parameterized by~{#1}}%
            }
        \begin{tabular*}{\textwidth}{@{\hspace{.1em}} >{\itshape} p{1.8cm} p{0.8\textwidth} @{}}%
    }{
        \end{tabular*}%
        \end{GrayBox}%
        \ignorespacesafterend
    }


\newcommand{\defproblema}[3]{%
    \begin{defproblemx}{#1}
    {\bf Instance:}  & #2 \\
    {\bf Goal:} & #3
    \end{defproblemx}
}%


\newcommand{\problemdef}[3]{\defproblema{#1}{#2}{#3}}
\newcommand{\revised}[1]{\textcolor{blue}{#1}}
